PointSAM: Pointly-Supervised Segment Anything Model for Remote Sensing Images

Segment Anything Model (SAM) is an advanced foundational model for image segmentation, which is gradually being applied to remote sensing images (RSIs). Due to the domain gap between RSIs and natural images, traditional methods typically use SAM as a source pre-trained model and fine-tune it with fully supervised masks. Unlike these methods, our work focuses on fine-tuning SAM using more convenient and challenging point annotations. Leveraging SAM's zero-shot capabilities, we adopt a self-training framework that iteratively generates pseudo-labels for training. However, if the pseudo-labels contain noisy labels, there is a risk of error accumulation. To address this issue, we extract target prototypes from the target dataset and use the Hungarian algorithm to match them with prediction prototypes, preventing the model from learning in the wrong direction. Additionally, due to the complex backgrounds and dense distribution of objects in RSI, using point prompts may result in multiple objects being recognized as one. To solve this problem, we propose a negative prompt calibration method based on the non-overlapping nature of instance masks. In brief, we use the prompts of overlapping masks as corresponding negative signals, resulting in refined masks. Combining the above methods, we propose a novel Pointly-supervised Segment Anything Model named PointSAM. We conduct experiments on RSI datasets, including WHU, HRSID, and NWPU VHR-10, and the results show that our method significantly outperforms direct testing with SAM, SAM2, and other comparison methods. Furthermore, we introduce PointSAM as a point-to-box converter and achieve encouraging results, suggesting that this method can be extended to other point-supervised tasks. The code is available at https://github.com/Lans1ng/PointSAM.

==> pic/sam.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,492); %set diagram left start at 0, and has height of 492

%Shape: Trapezoid [id:dp517137829898388] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 251; green, 229; blue, 224 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (122.14,48) -- (170.48,58.28) -- (170.48,87.72) -- (122.14,98) -- cycle ;
%Shape: Trapezoid [id:dp7015064236451118] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 231; blue, 253 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (246.48,49.24) -- (198.14,59.52) -- (198.14,88.96) -- (246.48,99.24) -- cycle ;
%Rounded Rect [id:dp11325921632007652] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 226; green, 239; blue, 216 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (196.22,123.96) .. controls (196.22,120.48) and (199.04,117.67) .. (202.51,117.67) -- (247.27,117.67) .. controls (250.74,117.67) and (253.56,120.48) .. (253.56,123.96) -- (253.56,142.82) .. controls (253.56,146.3) and (250.74,149.11) .. (247.27,149.11) -- (202.51,149.11) .. controls (199.04,149.11) and (196.22,146.3) .. (196.22,142.82) -- cycle ;
%Straight Lines [id:da8301104884179427] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (98.48,73.5) -- (111.42,73.5) ;
\draw [shift={(115.42,73.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da8801256610079162] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (260.38,134) -- (273.32,134) ;
\draw [shift={(256.38,134)}, rotate = 0] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da37115817274359597] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (176.08,73.5) -- (189.02,73.5) ;
\draw [shift={(193.02,73.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da4867810918187998] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (248.88,73.5) -- (261.82,73.5) ;
\draw [shift={(265.82,73.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da6805481378139688] 
\draw [color={rgb, 255:red, 238; green, 156; blue, 133 }  ,draw opacity=1 ][line width=1.5]    (315.68,73.5) -- (328.62,73.5) ;
\draw [shift={(311.68,73.5)}, rotate = 0] [fill={rgb, 255:red, 238; green, 156; blue, 133 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da44738145178819355] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (224.48,113) -- (224.48,101.87) ;
\draw [shift={(224.48,97.87)}, rotate = 90] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Shape: Trapezoid [id:dp7512612245397305] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 251; green, 229; blue, 224 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (122.14,171) -- (170.48,181.28) -- (170.48,210.72) -- (122.14,221) -- cycle ;
%Shape: Trapezoid [id:dp9101838846284189] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 231; blue, 253 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (246.48,172.24) -- (198.14,182.52) -- (198.14,211.96) -- (246.48,222.24) -- cycle ;
%Rounded Rect [id:dp4248968686833223] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 226; green, 239; blue, 216 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (196.22,246.96) .. controls (196.22,243.48) and (199.04,240.67) .. (202.51,240.67) -- (247.27,240.67) .. controls (250.74,240.67) and (253.56,243.48) .. (253.56,246.96) -- (253.56,265.82) .. controls (253.56,269.3) and (250.74,272.11) .. (247.27,272.11) -- (202.51,272.11) .. controls (199.04,272.11) and (196.22,269.3) .. (196.22,265.82) -- cycle ;
%Straight Lines [id:da10684056515743312] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (98.48,196.5) -- (111.42,196.5) ;
\draw [shift={(115.42,196.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da6201155079183256] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (260.38,257) -- (273.32,257) ;
\draw [shift={(256.38,257)}, rotate = 0] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da47701466082781785] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (176.08,196.5) -- (189.02,196.5) ;
\draw [shift={(193.02,196.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da7338990416665101] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (248.88,196.5) -- (261.82,196.5) ;
\draw [shift={(265.82,196.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da3105456300598102] 
\draw [color={rgb, 255:red, 238; green, 156; blue, 133 }  ,draw opacity=1 ][line width=1.5]    (315.68,196.5) -- (328.62,196.5) ;
\draw [shift={(311.68,196.5)}, rotate = 0] [fill={rgb, 255:red, 238; green, 156; blue, 133 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da4253468031471981] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (224.48,236) -- (224.48,224.87) ;
\draw [shift={(224.48,220.87)}, rotate = 90] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Rounded Rect [id:dp5708398454570627] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (108.17,239.32) .. controls (108.17,237.21) and (109.87,235.51) .. (111.98,235.51) -- (179.35,235.51) .. controls (181.46,235.51) and (183.17,237.21) .. (183.17,239.32) -- (183.17,262.2) .. controls (183.17,264.3) and (181.46,266.01) .. (179.35,266.01) -- (111.98,266.01) .. controls (109.87,266.01) and (108.17,264.3) .. (108.17,262.2) -- cycle ;
%Shape: Cross [id:dp3731313502739675] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (145.08,219) -- (147.25,219) -- (147.25,224.42) -- (152.67,224.42) -- (152.67,226.58) -- (147.25,226.58) -- (147.25,232) -- (145.08,232) -- (145.08,226.58) -- (139.67,226.58) -- (139.67,224.42) -- (145.08,224.42) -- cycle ;
%Shape: Rectangle [id:dp9712050208027316] 
\draw   (113.83,238.5) -- (136.83,238.5) -- (136.83,261.5) -- (113.83,261.5) -- cycle ;
%Shape: Rectangle [id:dp28477060038772595] 
\draw   (155.67,238.5) -- (178.67,238.5) -- (178.67,261.5) -- (155.67,261.5) -- cycle ;
%Shape: Cross [id:dp5762472319237713] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (149.53,244.14) -- (151.06,245.67) -- (147.23,249.5) -- (151.06,253.33) -- (149.53,254.86) -- (145.7,251.03) -- (141.87,254.86) -- (140.34,253.33) -- (144.17,249.5) -- (140.34,245.67) -- (141.87,244.14) -- (145.7,247.97) -- cycle ;
%Straight Lines [id:da6330587392134064] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (71,160.67) -- (364.33,160.67) ;
%Straight Lines [id:da25313290359179597] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (71,287.33) -- (364.33,287.33) ;
%Shape: Trapezoid [id:dp7230421260043707] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 251; green, 229; blue, 224 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (124.8,299) -- (173.14,309.28) -- (173.14,338.72) -- (124.8,349) -- cycle ;
%Shape: Trapezoid [id:dp06695037168776352] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 231; blue, 253 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (249.14,300.24) -- (200.8,310.52) -- (200.8,339.96) -- (249.14,350.24) -- cycle ;
%Rounded Rect [id:dp054124074932860644] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][fill={rgb, 255:red, 226; green, 239; blue, 216 }  ,fill opacity=1 ][blur shadow={shadow xshift=0pt,shadow yshift=0pt, shadow blur radius=0.75pt, shadow blur steps=4 ,shadow opacity=100}] (198.89,374.96) .. controls (198.89,371.48) and (201.7,368.67) .. (205.18,368.67) -- (249.93,368.67) .. controls (253.41,368.67) and (256.22,371.48) .. (256.22,374.96) -- (256.22,393.82) .. controls (256.22,397.3) and (253.41,400.11) .. (249.93,400.11) -- (205.18,400.11) .. controls (201.7,400.11) and (198.89,397.3) .. (198.89,393.82) -- cycle ;
%Straight Lines [id:da6667979612465196] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (102.48,309.17) -- (115.42,309.17) ;
\draw [shift={(119.42,309.17)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da37970099149254244] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (263.04,385) -- (275.99,385) ;
\draw [shift={(259.04,385)}, rotate = 0] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da16912613846384494] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (178.74,324.5) -- (191.69,324.5) ;
\draw [shift={(195.69,324.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da05081847658875871] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (255.68,308.5) -- (268.62,308.5) ;
\draw [shift={(272.62,308.5)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da38467847370910846] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (227.14,364) -- (227.14,352.87) ;
\draw [shift={(227.14,348.87)}, rotate = 90] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da6332908179981049] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (103.14,339.17) -- (116.09,339.17) ;
\draw [shift={(120.09,339.17)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da8978766572674732] 
\draw [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ][line width=1.5]    (255.68,337.83) -- (268.62,337.83) ;
\draw [shift={(272.62,337.83)}, rotate = 180] [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Curve Lines [id:da8790517923424956] 
\draw [color={rgb, 255:red, 238; green, 156; blue, 133 }  ,draw opacity=1 ][line width=1.5]    (323,306.26) .. controls (339.36,312.88) and (340.72,331.67) .. (325.43,340.15) ;
\draw [shift={(322,341.76)}, rotate = 338.5] [fill={rgb, 255:red, 238; green, 156; blue, 133 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (6.97,-3.35) -- (0,0) -- (6.97,3.35) -- cycle    ;
%Straight Lines [id:da06422058954897314] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (71,408.33) -- (364.33,408.33) ;

% Text Node
\draw (148.97,324) node   [align=left] {\begin{minipage}[lt]{36.92pt}\setlength\topsep{0pt}
\begin{center}
{\small Image }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (227.56,384.39) node   [align=left] {\begin{minipage}[lt]{36.92pt}\setlength\topsep{0pt}
\begin{center}
{\small Prompt }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (224.97,325.24) node   [align=left] {\begin{minipage}[lt]{37.42pt}\setlength\topsep{0pt}
\begin{center}
{\small Mask }\\{\small Decoder}
\end{center}

\end{minipage}};
% Text Node
\draw (73,300.57) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{I}_{img}$};
% Text Node
\draw (276.33,300.57) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}_{pred}$};
% Text Node
\draw (280.33,378.23) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{P}$};
% Text Node
\draw (73.67,330.57) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{I}^\prime _{img}$};
% Text Node
\draw (277.67,329.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}^\prime _{pred}$};
% Text Node
\draw (146.31,196) node   [align=left] {\begin{minipage}[lt]{36.92pt}\setlength\topsep{0pt}
\begin{center}
{\small Image }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (224.89,256.39) node   [align=left] {\begin{minipage}[lt]{36.92pt}\setlength\topsep{0pt}
\begin{center}
{\small Prompt }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (222.31,197.24) node   [align=left] {\begin{minipage}[lt]{37.42pt}\setlength\topsep{0pt}
\begin{center}
{\small Mask }\\{\small Decoder}
\end{center}

\end{minipage}};
% Text Node
\draw (69,187.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{I}_{img}$};
% Text Node
\draw (334.47,187.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}_{gt}$};
% Text Node
\draw (267.67,187.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}_{pred}$};
% Text Node
\draw (277.67,250.23) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{P}$};
% Text Node
\draw (125.33,250) node   [align=left] {$\displaystyle A$};
% Text Node
\draw (167.17,250) node   [align=left] {$\displaystyle B$};
% Text Node
\draw (146.31,73) node   [align=left] {\begin{minipage}[lt]{33.3pt}\setlength\topsep{0pt}
\begin{center}
{\small {\fontfamily{ptm}\selectfont Image }}\\{\small {\fontfamily{ptm}\selectfont Encoder}}
\end{center}

\end{minipage}};
% Text Node
\draw (224.89,133.39) node   [align=left] {\begin{minipage}[lt]{36.92pt}\setlength\topsep{0pt}
\begin{center}
{\small Prompt }\\{\small Encoder}
\end{center}

\end{minipage}};
% Text Node
\draw (222.31,74.24) node   [align=left] {\begin{minipage}[lt]{37.42pt}\setlength\topsep{0pt}
\begin{center}
{\small Mask }\\{\small Decoder}
\end{center}

\end{minipage}};
% Text Node
\draw (69,64.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{I}_{img}$};
% Text Node
\draw (334.47,64.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}_{gt}$};
% Text Node
\draw (267.67,64.9) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{M}_{pred}$};
% Text Node
\draw (277.67,127.23) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{P}$};
% Text Node
\draw (73,157.67) node [anchor=south west] [inner sep=0.75pt]   [align=left] {\textbf{(a) SAM}};
% Text Node
\draw (73,284.33) node [anchor=south west] [inner sep=0.75pt]   [align=left] {\textbf{(b) LoRA}};
% Text Node
\draw (73,405.33) node [anchor=south west] [inner sep=0.75pt]   [align=left] {\textbf{(c) Self Training}};


\end{tikzpicture}

